Signatures of extended radio emission from escaping electrons in the Lighthouse Nebula

Several supersonic runaway pulsar wind nebulae (sPWNe) with jet-like extended structures have been recently discovered in X-rays. If these structures are the product of electrons escaping the system and diffusing into the surrounding interstellar medium, they can produce a radio halo extending for several arcmin around the source. We model the expected radio emission in this scenario in the Lighthouse Nebula sPWN. We assume a constant particle injection rate during the source lifetime, and isotropic diffusion into the surrounding medium. Our predictions strongly depend on the low- and high-energy cutoffs given in the particle distribution. Our results indicate that extended radio emission can be detected from the Lighthouse Nebula without the need to invoke extreme values for the model parameters. We provide synthetic synchrotron maps that can be used to constrain these results with observations by current highly sensitive radio instruments.

==> arXiv submission/FIGURES/Fig1_sketch.tex <==
% %________________________________________________________________________
% %\begin{comment}
% \begin{figure}[t]
% %
% \centering
% \includegraphics{FIGURES/LN_sketch_v3.pdf}
% caption{
% Chandra/ACIS exposure-corrected 0.5 -- 7.0 keV image of IGR J11014–6103 (the “Lighthouse nebula”).The image has a pixel size of 0.492$\arcsec$ and has been smoothed with a 2D-Gaussian kernel with a radius of 2.2$\arcsec$.
%   }
%  \label{figure:sketch}
% \end{figure}

%_____________________________________________________________________


\begin{figure}[h]
  \centering
    \includegraphics[width=0.5\textwidth]{FIGURES/LN_sketch_v2b.pdf}
  \caption{\textit{Chandra}/ACIS exposure-corrected broadband (0.5 -- 7.0 keV) flux image of IGR J11014–6103 (the ``Lighthouse Nebula''). The image has been produced using all \textit{Chandra} archival observations of the \lneb, for a total of $\sim365$~ks, merged using CIAO's {\texttt{merge\_obs}} tool, and smoothed using a 2D Gaussian kernel with radius  on a pixel size of 0.492$\arcsec$ and has been smoothed with a 2D-Gaussian kernel with radius = 1.7$\arcsec$ and $\sigma = 0.7$\arcsec.}
  \label{figure:sketch}
\end{figure}

==> arXiv submission/FIGURES/Fig2_distributions.tex <==

%________________________________________________________________________
\begin{figure}[t]
\centering
%\includegraphics[width=0.5\textwidth]{FIGURES/distributions_gmin1e3.pdf}
\includegraphics[width=0.5\textwidth]{FIGURES/distros_2cuts.pdf}
\caption{Energy distribution of non-thermal particles injected into the JET and ISM regions for different assumed values of the low-energy cutoff $\gamma_{\rm min}^{cut}$. Particle injection is discretized as occurring every $t_{\rm inj} = 1$~kyr (dotted lines). The final cumulative distribution at present time accounts for radiation cooling due to IC on the CMB and synchrotron losses. Distributions are shown for particles injected recently ($t_{\rm inj} \leq 1$~kyr) that diffuse through the JET region (blue lines), and particles injected at $t_{\rm inj} > 1$~kyr diffusing into the ISM region (in red lines). In both cases, a magnetic field of $B_{\rm ISM} = B_{\rm JET} = 5\mu$G is assumed. A low cutoff for the particle distribution at injection is considered, adopting two different values $\gamma_{\rm min}^{cut} = 10^{3}$  and $\gamma_{\rm min}^{cut} = 10^{5}$ (solid and dashed lines, respectively). A high energy cutoff $\gamma_{\rm max}^{cut} = 10^{8}$ is also assumed in all cases. The distribution normalization is computed accounting for the source observed X-ray luminosity (see text for details).}
\label{figure:particle_distribution}
\end{figure}
%________________________________________________________________________

==> arXiv submission/FIGURES/Fig3_SEDs.tex <==
%________________________________________________________________________
%\begin{comment}
\begin{figure*}[t]
%
 \begin{subfigure}{.5\textwidth}
   \centering
   \includegraphics[width=0.95\textwidth]{FIGURES/SED_and_limits_gmin1e3_nuLnu}
   \end{subfigure}%
 %
 \begin{subfigure}{.5\textwidth}
   \centering
   \includegraphics[width=0.95\textwidth]{FIGURES/SED_and_limits_gmin1e5_nuLnu}
   \end{subfigure}
 %  
  \caption{
  \textbf{Left}: Spectral energy distribution of the emission produced by electrons injected in the ISM (in red) and JET regions (in blue). A magnetic field $B_{\rm ISM} = 5\mu$G is assumed for the ISM, whereas a range in the value of $B_{\rm JET} = 5, 10, 15, 20$ and $30\mu$G is probed for the JET region. Particle injection is considered up to $t_{\rm inj} = 10^3$~yr for the JET region and from $t_{\rm inj} = 10^3$~yr until $t_{\rm inj} = 20$~kyr for the ISM region (red-dotted lines). Particles are assumed to follow a power-law distribution with a low and a high energy cutoff $\gamma_{\rm min}^{cut} = 10^{3}$ and $\gamma_{\rm max}^{cut} = 10^{8}$, respectively. Green and orange vertical bands denote \textit{Chandra} and MeerKAT frequency coverage. \textbf{Right}: Same as in the left panel but for a particle spectrum with a low-energy cutoff $\gamma_{\rm min}^{cut} = 10^{5}$.
  }
 \label{figure:SEDs}
\end{figure*}
%\end{comment}
%_____________________________________________________________________

==> arXiv submission/FIGURES/Fig4_maps.tex <==
%_____________________________________________________________________

%\begin{comment}
\begin{figure*}[t]
%
 \begin{subfigure}{.5\textwidth}
   \centering
   \includegraphics[width=\linewidth]{FIGURES/maps_ISM_gmin1e3.png}
   \end{subfigure}%
 %
 \begin{subfigure}{.5\textwidth}
   \centering
   \includegraphics[width=\linewidth]{FIGURES/maps_JET_gmin1e3.png}
   \end{subfigure}
 %  
  \caption
    {Synthetic synchrotron specific flux maps displaying the expected radio emission from \igr in the 0.9--1.7 GHz band in which MeerKAT operates, convolved with an instrument beam of $15\arcsec \times 15\arcsec$ (\citealp{Jonas2016}). The contribution from particles injected all along the \IGR's lifetime, which escaped the nebula and diffused into the ISM ($B_{\rm ISM} = 5\mu$G), is displayed in the left panel, and that from the JET region ($B_{\rm ISM} = 30\mu$G) is shown in the right panel. A white star indicates the position of the pulsar, which is assumed to move leftwards along the horizontal dashed-line. }
\label{figure:maps_gmin1e3}
\end{figure*}


%\end{comment}
%________________________________________________________________________
